Snips Voice Platform: an embedded Spoken Language Understanding system for private-by-design voice interfaces

This paper presents the machine learning architecture of the Snips Voice Platform, a software solution to perform Spoken Language Understanding on microprocessors typical of IoT devices. The embedded inference is fast and accurate while enforcing privacy by design, as no personal user data is ever collected. Focusing on Automatic Speech Recognition and Natural Language Understanding, we detail our approach to training high-performance Machine Learning models that are small enough to run in real-time on small devices. Additionally, we describe a data generation procedure that provides sufficient, high-quality training data without compromising user privacy.

==> sec_ccl.tex <==
\section{Conclusion and future work}
Snips offers a fully embedded Voice Platform. All of our inference algorithms, which run on common IoT devices, are trained on servers on data that we generate, before they are deployed, without requiring any user data. As is, Snips solution is a first working implementation of decentralized machine learning. In the coming months, we plan on publishing a benchmark for the complete Spoken Language Understanding solution, comparing to the main cloud-based alternatives. We are currently researching partially homomorphic encrypted analytics to improve feedback from our users and exploring federated learning as a mean to replace data generation while maintaining privacy.
